Metal Inter-layer Via Keep-out-zone in M3D IC: A Critical Process-aware Design Consideration

Metal inter-layer via (MIV) in Monolithic three-dimensional integrated circuits (M3D-IC) is used to connect inter-layer devices and provide power and clock signals across multiple layers. The size of MIV is comparable to logic gates because of the significant reduction in substrate layers due to sequential integration. Despite MIV's small size, the impact of MIV on the performance of adjacent devices should be considered to implement IC designs in M3D-IC technology. In this work, we systematically study the changes in performance of transistors when they are placed near MIV to understand the effect of MIV on adjacent devices when MIV passes through the substrate. Simulation results suggest that the keep-out-zone (KOZ) for MIV should be considered to ensure the reliability of M3D-IC technology and this KOZ is highly dependent on the M3D-IC process. In this paper, we show that the transistor placed near MIV considering the M1 metal pitch as the separation will have up to $68,668\times$ increase in leakage current, when the channel doping is $10^{15} cm^{-3}$, source/drain doping of $10^{18}cm^{-3}$ and substrate layer height of $100\ nm$. We also show that, this increase in leakage current can also be reduced significantly by having KOZ around MIV, which is dependent on the process.

==> Section_background_notused.tex <==
\section{Background and Motivation}\label{sec:background}

==> check.tex <==

\begin{table*}[htp]
    \centering
   \caption{Process variation and MIV separation effect on transistor performance}\label{tab:process_variations}
   \scalebox{0.65}{
    \begin{NiceTabular}{|c|c|c|l|l|l|l|l|l|l|l|c|}
         \hline
          & $n_{src} $ & $n_{sub} $ & \multicolumn{2}{c|}{$H_{sub}=25 nm$}& \multicolumn{2}{c|}{$H_{sub}=50 nm$} & \multicolumn{2}{c|}{$H_{sub}=75 nm$}& \multicolumn{2}{c|}{$H_{sub}=100 nm$} & \multirow{2}{*}{Case} \\ \cline{4-11} 
        \textbf {} & $(cm^{-3})$ &  $(cm^{-3})$ & \multicolumn{1}{|c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{|c|}{$I_{leak} \ (A)$} 
        & \multicolumn{1}{|c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{|c|}{$I_{leak} \ (A)$}
        & \multicolumn{1}{|c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{|c|}{$I_{leak} \ (A)$}
        & \multicolumn{1}{|c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{|c|}{$I_{leak} \ (A)$} & \\
        \hline 
        \multirow{8}{*}{\rotatebox{90}{$d_{sep}=50nm$}}
        & \multirow{2}{*}{1E18} 
    %   nsub % Imax_with_MIV % Ileak_withMIV
        & 1E15
                % hsub=25nm
               
                &  \bc $4.60\ (\times1.30)$ & \bc $1.65\times10^{-07}\ (\times171)$ 
                % hsub=50nm
                & \bc $4.48\ (\times1.64)$ & \bc $2.63\times10^{-07}\ (\times882)$
                % hsub=75nm
                & \bc $4.66\ (\times2.01)$ & \bc $3.04\times10^{-07}\ (\times8090)$
                % hsub=100nm
                & \bc $4.55\ (\times2.53)$ & \bc $3.50\times10^{-07}\ (\times68668)$  & 1 \\ \cline{3-12}
        
        & & 1E16
                % hsub=25nm
                & $2.89\ (\times2.00)$ & \cellcolor{green_t} $5.34\times10^{-09}\ (\times1865)$ 
                % hsub=50nm
                & $1.71\ (\times3.30)$ & \cellcolor{green_t} $1.01\times10^{-09}\ (\times13906)$
                % hsub=75nm
                & $1.45\ (\times5.90)$ & \cellcolor{green_t} $4.56\times10^{-10}\ (\times31241)$
                % hsub=100nm
                & $1.30\ (\times6.53)$ & \cellcolor{green_t} $3.10\times10^{-10}\ (\times44983)$ & \multirow{2}{*}{2} \\ \cline{4-11}
        

        \cline{2-3}
        & \multirow{2}{*}{1E19} 
        & 1E16   
                % hsub=25nm
                & $11.89\ (\times1.29)$ & \cellcolor{green_t} $8.93\times10^{-08}\ (\times442)$ 
                % hsub=50nm
                & $9.34\ (\times1.56)$ & \cellcolor{green_t} $1.25\times10^{-08}\ (\times6988)$
                % hsub=75nm
                & $8.23\ (\times1.84)$ & \cellcolor{green_t} $5.00\times10^{-09}\ (\times18709)$
                % hsub=100nm
                & $7.92\ (\times1.90)$ & \cellcolor{green_t} $2.83\times10^{-09}\ (\times31175)$ &  \\ \cline{3-12}
          
        
        & & 1E17
                % hsub=25nm
                &  \pc $8.57\ (\times1.33)$ & \pc $1.78\times10^{-10}\ (\times244)$ 
                % hsub=50nm
                & \pc $5.37\ (\times1.56)$ &  \pc $1.33\times10^{-12}\ (\times201)$
                % hsub=75nm
                & \pc $4.51\ (\times1.59)$ & \pc $4.61\times10^{-13}\ (\times99)$
                % hsub=100nm
                & \pc $4.35\ (\times1.56)$ & \pc $2.64\times10^{-13}\ (\times70)$ & 3 \\ \cline{4-12}
        
        

        \cline{2-3}
        & \multirow{2}{*}{1E20} 
        & 1E17   
                % hsub=25nm
                & \cellcolor{grey_t} $30.60\ (\times1.12)$ & $8.23\times10^{-07}\ (\times7)$ 
                % hsub=50nm
                & \cellcolor{grey_t} $24.92\ (\times1.15)$ & $2.15\times10^{-08}\ (\times26)$
                % hsub=75nm
                & \cellcolor{grey_t} $23.51\ (\times1.16)$ & $8.51\times10^{-09}\ (\times26)$
                % hsub=100nm
                & \cellcolor{grey_t} $23.24\ (\times1.15)$ & $3.74\times10^{-09}\ (\times17)$ & 4 \\ \cline{3-12}
        
        & & 1E18 
                % hsub=25nm
                & \yc $17.89\ (\times1.01)$ & \yc $3.36\times10^{-11}\ (\times1.13)$ 
                % hsub=50nm
                & \yc  $14.92\ (\times1.00)$ & \yc $2.63\times10^{-12}\ (\times1.09)$
                % hsub=75nm
                & \yc $14.81\ (\times1.01)$ & \yc $2.35\times10^{-12}\ (\times1.21)$
                % hsub=100nm
                & \yc $15.09\ (\times1.01)$ & \yc $2.41\times10^{-12}\ (\times1.07)$ & \multirow{3}{*}{5}\\ \cline{4-11}
        
        \cline{2-3}
        
        & \multirow{2}{*}{1E21} 
        & 1E18   
                % hsub=25nm
                & \yc $29.21\ (\times1.02)$ & \yc $3.60\times10^{-08}\ (\times1.16)$ 
                % hsub=50nm
                & \yc $24.61\ (\times1.02)$ & \yc $2.37\times10^{-09}\ (\times1.20)$
                % hsub=75nm
                & \yc $24.36\ (\times1.01)$ & \yc $2.25\times10^{-09}\ (\times1.10)$
                % hsub=100nm
                & \yc $24.93\ (\times1.01)$ & \yc $3.60\times10^{-09}\ (\times1.09)$ &  \\ \cline{3-11}
        
        & & 1E19 
                % hsub=25nm
                & \yc $4.01\ (\times1.03)$ & \yc $3.79\times10^{-15}\ (\times1.16)$ 
                % hsub=50nm
                & \yc $4.01\ (\times1.02)$ & \yc $4.45\times10^{-15}\ (\times1.13)$
                % hsub=75nm
                & \yc $3.47\ (\times1.00)$ & \yc $3.01\times10^{-15}\ (\times1.03)$
                % hsub=100nm
                & \yc $4.32\ (\times1.00)$ & \yc $6.39\times10^{-15}\ (\times1.00)$ &  \\ \cline{4-12}
        

        
        \hline \hline
        
        \multirow{5}{*}{\rotatebox{90}{$d_{sep}=100nm$}}
        & \multirow{2}{*}{1E18} 
    %   nsub % Imax_with_MIV % Ileak_withMIV
        & 1E15
                % hsub=25nm
                &  \bc $4.31\ (\times1.22)$ & \bc $4.54\times10^{-08}\ (\times47)$ 
                % hsub=50nm
                & \bc $4.02\ (\times1.47)$ &  \bc $7.08\times10^{-08}\ (\times237)$
                % hsub=75nm
                & \bc $4.00\ (\times1.72)$ & \bc $7.40\times10^{-08}\ (\times1971)$
                % hsub=100nm
                & \bc $3.84\ (\times2.13)$ & \bc $8.07\times10^{-08}\ (\times15839)$ & 1 \\ \cline{3-12}
        
        & & 1E16
                % hsub=25nm
                & $2.48\ (\times1.72)$ & \cellcolor{green_t} $3.51\times10^{-10}\ (\times123)$ 
                % hsub=50nm
                & $1.22\ (\times2.36)$ & \cellcolor{green_t} $2.94\times10^{-11}\ (\times403)$
                % hsub=75nm
                & $0.89\ (\times3.62)$ & \cellcolor{green_t} $6.35\times10^{-12}\ (\times435)$
                % hsub=100nm
                & $0.73\ (\times3.66)$ & \cellcolor{green_t} $2.78\times10^{-12}\ (\times404)$ & \multirow{2}{*}{2} \\ 
                \cline{4-11}
        

        
        \cline{2-3}
        & \multirow{2}{*}{1E19} 
        & 1E16   
                % hsub=25nm
                & $11.23\ (\times1.22)$ & \cellcolor{green_t} $1.23\times10^{-08}\ (\times61)$ 
                % hsub=50nm
                & $8.24\ (\times1.37)$ & \cellcolor{green_t} $5.11\times10^{-10}\ (\times285)$
                % hsub=75nm
                & $6.86\ (\times1.54)$ & \cellcolor{green_t} $8.28\times10^{-11}\ (\times310)$
                % hsub=100nm
                & $6.43\ (\times1.54)$ & \cellcolor{green_t} $2.75\times10^{-11}\ (\times303)$ &  \\ \cline{3-12}
          
        % edit from here
        & & 1E17
                % hsub=25nm
                &  \pc $7.33\ (\times1.13)$ & \pc $2.84\times10^{-12}\ (\times4)$ 
                % hsub=50nm
                & \pc $3.76\ (\times1.09)$ & \pc $1.32\times10^{-14}\ (\times2)$
                % hsub=75nm
                & \pc $3.15\ (\times1.12)$ & \pc $7.01\times10^{-15}\ (\times2)$
                % hsub=100nm
                & \pc $3.01\ (\times1.08)$ & \pc $5.31\times10^{-15}\ (\times1.41)$ & 3 \\ \cline{3-12}
        

        \cline{2-11}
        & \multirow{1}{*}{1E20} 
        & 1E17   
                % hsub=25nm
                & \cellcolor{grey_t} $28.87\ (\times1.06)$ & $2.79\times10^{-07}\ (\times2)$ 
                % hsub=50nm
                & \cellcolor{grey_t} $22.61\ (\times1.05)$ & $2.08\times10^{-09}\ (\times3)$
                % hsub=75nm
                & \cellcolor{grey_t} $21.19\ (\times1.04)$ & $7.04\times10^{-10}\ (\times2)$
                % hsub=100nm
                & \cellcolor{grey_t} $21.02\ (\times1.04)$ & $3.75\times10^{-10}\ (\times2)$ & 4 \\
        
        \hline 
        
    \end{NiceTabular} 
    }
\end{table*}

==> dummy/section5_table_backup.tex <==
\begin{table*}[htp]
    \centering
   \caption{Process variation and MIV separation effect on transistor performance}\label{tab:process_variations}
   \scalebox{0.65}{
    \begin{NiceTabular}{|c|c|c|l|l|l|l|l|l|l|l|c|}
         \hline
          & $n_{src} $ & $n_{sub} $ & \multicolumn{2}{c|}{$H_{sub}=25 nm$}& \multicolumn{2}{c|}{$H_{sub}=50 nm$} & \multicolumn{2}{c|}{$H_{sub}=75 nm$}& \multicolumn{2}{c|}{$H_{sub}=100 nm$} & \multirow{2}{*}{Case} \\ \cline{4-11} 
        \textbf {} & $(cm^{-3})$ &  $(cm^{-3})$ & \multicolumn{1}{|c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{|c|}{$I_{leak} \ (A)$} 
        & \multicolumn{1}{|c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{|c|}{$I_{leak} \ (A)$}
        & \multicolumn{1}{|c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{|c|}{$I_{leak} \ (A)$}
        & \multicolumn{1}{|c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{|c|}{$I_{leak} \ (A)$} & \\
        \hline 
        \multirow{8}{*}{\rotatebox{90}{$d_{sep}=50nm$}}
        & \multirow{2}{*}{1E18} 
    %   nsub % Imax_with_MIV % Ileak_withMIV
        & 1E15
                % hsub=25nm
               
                &  \bc $4.60\ (\times1.30)$ & \bc $1.65\times10^{-07}\ (\times171)$ 
                % hsub=50nm
                & \bc $4.48\ (\times1.64)$ & \bc $2.63\times10^{-07}\ (\times882)$
                % hsub=75nm
                & \bc $4.66\ (\times2.01)$ & \bc $3.04\times10^{-07}\ (\times8090)$
                % hsub=100nm
                & \bc $4.55\ (\times2.53)$ & \bc $3.50\times10^{-07}\ (\times68668)$  & 1 \\ \cline{3-12}
        
        & & 1E16
                % hsub=25nm
                & $2.89\ (\times2.00)$ & \cellcolor{green_t} $5.34\times10^{-09}\ (\times1865)$ 
                % hsub=50nm
                & $1.71\ (\times3.30)$ & \cellcolor{green_t} $1.01\times10^{-09}\ (\times13906)$
                % hsub=75nm
                & $1.45\ (\times5.90)$ & \cellcolor{green_t} $4.56\times10^{-10}\ (\times31241)$
                % hsub=100nm
                & $1.30\ (\times6.53)$ & \cellcolor{green_t} $3.10\times10^{-10}\ (\times44983)$ & \multirow{2}{*}{2} \\ \cline{4-11}
        

        \cline{2-3}
        & \multirow{2}{*}{1E19} 
        & 1E16   
                % hsub=25nm
                & $11.89\ (\times1.29)$ & \cellcolor{green_t} $8.93\times10^{-08}\ (\times442)$ 
                % hsub=50nm
                & $9.34\ (\times1.56)$ & \cellcolor{green_t} $1.25\times10^{-08}\ (\times6988)$
                % hsub=75nm
                & $8.23\ (\times1.84)$ & \cellcolor{green_t} $5.00\times10^{-09}\ (\times18709)$
                % hsub=100nm
                & $7.92\ (\times1.90)$ & \cellcolor{green_t} $2.83\times10^{-09}\ (\times31175)$ &  \\ \cline{3-12}
          
        
        & & 1E17
                % hsub=25nm
                &  \pc $8.57\ (\times1.33)$ & \pc $1.78\times10^{-10}\ (\times244)$ 
                % hsub=50nm
                & \pc $5.37\ (\times1.56)$ &  \pc $1.33\times10^{-12}\ (\times201)$
                % hsub=75nm
                & \pc $4.51\ (\times1.59)$ & \pc $4.61\times10^{-13}\ (\times99)$
                % hsub=100nm
                & \pc $4.35\ (\times1.56)$ & \pc $2.64\times10^{-13}\ (\times70)$ & 3 \\ \cline{4-12}
        
        

        \cline{2-3}
        & \multirow{2}{*}{1E20} 
        & 1E17   
                % hsub=25nm
                & \cellcolor{grey_t} $30.60\ (\times1.12)$ & $8.23\times10^{-07}\ (\times7)$ 
                % hsub=50nm
                & \cellcolor{grey_t} $24.92\ (\times1.15)$ & $2.15\times10^{-08}\ (\times26)$
                % hsub=75nm
                & \cellcolor{grey_t} $23.51\ (\times1.16)$ & $8.51\times10^{-09}\ (\times26)$
                % hsub=100nm
                & \cellcolor{grey_t} $23.24\ (\times1.15)$ & $3.74\times10^{-09}\ (\times17)$ & 4 \\ \cline{3-12}
        
        & & 1E18 
                % hsub=25nm
                & \yc $17.89\ (\times1.01)$ & \yc $3.36\times10^{-11}\ (\times1.13)$ 
                % hsub=50nm
                & \yc  $14.92\ (\times1.00)$ & \yc $2.63\times10^{-12}\ (\times1.09)$
                % hsub=75nm
                & \yc $14.81\ (\times1.01)$ & \yc $2.35\times10^{-12}\ (\times1.21)$
                % hsub=100nm
                & \yc $15.09\ (\times1.01)$ & \yc $2.41\times10^{-12}\ (\times1.07)$ & \multirow{3}{*}{5}\\ \cline{4-11}
        
        \cline{2-3}
        
        & \multirow{2}{*}{1E21} 
        & 1E18   
                % hsub=25nm
                & \yc $29.21\ (\times1.02)$ & \yc $3.60\times10^{-08}\ (\times1.16)$ 
                % hsub=50nm
                & \yc $24.61\ (\times1.02)$ & \yc $2.37\times10^{-09}\ (\times1.20)$
                % hsub=75nm
                & \yc $24.36\ (\times1.01)$ & \yc $2.25\times10^{-09}\ (\times1.10)$
                % hsub=100nm
                & \yc $24.93\ (\times1.01)$ & \yc $3.60\times10^{-09}\ (\times1.09)$ &  \\ \cline{3-11}
        
        & & 1E19 
                % hsub=25nm
                & \yc $4.01\ (\times1.03)$ & \yc $3.79\times10^{-15}\ (\times1.16)$ 
                % hsub=50nm
                & \yc $4.01\ (\times1.02)$ & \yc $4.45\times10^{-15}\ (\times1.13)$
                % hsub=75nm
                & \yc $3.47\ (\times1.00)$ & \yc $3.01\times10^{-15}\ (\times1.03)$
                % hsub=100nm
                & \yc $4.32\ (\times1.00)$ & \yc $6.39\times10^{-15}\ (\times1.00)$ &  \\ \cline{4-12}
        

        
        \hline 
        
        \iffalse
        \hline
        
        \multirow{5}{*}{\rotatebox{90}{$d_{sep}=100nm$}}
        & \multirow{2}{*}{1E18} 
    %   nsub % Imax_with_MIV % Ileak_withMIV
        & 1E15
                % hsub=25nm
                &  \bc $4.31\ (\times1.22)$ & \bc $4.54\times10^{-08}\ (\times47)$ 
                % hsub=50nm
                & \bc $4.02\ (\times1.47)$ &  \bc $7.08\times10^{-08}\ (\times237)$
                % hsub=75nm
                & \bc $4.00\ (\times1.72)$ & \bc $7.40\times10^{-08}\ (\times1971)$
                % hsub=100nm
                & \bc $3.84\ (\times2.13)$ & \bc $8.07\times10^{-08}\ (\times15839)$ & 1 \\ \cline{3-12}
        
        & & 1E16
                % hsub=25nm
                & $2.48\ (\times1.72)$ & \cellcolor{green_t} $3.51\times10^{-10}\ (\times123)$ 
                % hsub=50nm
                & $1.22\ (\times2.36)$ & \cellcolor{green_t} $2.94\times10^{-11}\ (\times403)$
                % hsub=75nm
                & $0.89\ (\times3.62)$ & \cellcolor{green_t} $6.35\times10^{-12}\ (\times435)$
                % hsub=100nm
                & $0.73\ (\times3.66)$ & \cellcolor{green_t} $2.78\times10^{-12}\ (\times404)$ & \multirow{2}{*}{2} \\ 
                \cline{4-11}
        

        
        \cline{2-3}
        & \multirow{2}{*}{1E19} 
        & 1E16   
                % hsub=25nm
                & $11.23\ (\times1.22)$ & \cellcolor{green_t} $1.23\times10^{-08}\ (\times61)$ 
                % hsub=50nm
                & $8.24\ (\times1.37)$ & \cellcolor{green_t} $5.11\times10^{-10}\ (\times285)$
                % hsub=75nm
                & $6.86\ (\times1.54)$ & \cellcolor{green_t} $8.28\times10^{-11}\ (\times310)$
                % hsub=100nm
                & $6.43\ (\times1.54)$ & \cellcolor{green_t} $2.75\times10^{-11}\ (\times303)$ &  \\ \cline{3-12}
          
        % edit from here
        & & 1E17
                % hsub=25nm
                &  \pc $7.33\ (\times1.13)$ & \pc $2.84\times10^{-12}\ (\times4)$ 
                % hsub=50nm
                & \pc $3.76\ (\times1.09)$ & \pc $1.32\times10^{-14}\ (\times2)$
                % hsub=75nm
                & \pc $3.15\ (\times1.12)$ & \pc $7.01\times10^{-15}\ (\times2)$
                % hsub=100nm
                & \pc $3.01\ (\times1.08)$ & \pc $5.31\times10^{-15}\ (\times1.41)$ & 3 \\ \cline{3-12}
        

        \cline{2-11}
        & \multirow{1}{*}{1E20} 
        & 1E17   
                % hsub=25nm
                & \cellcolor{grey_t} $28.87\ (\times1.06)$ & $2.79\times10^{-07}\ (\times2)$ 
                % hsub=50nm
                & \cellcolor{grey_t} $22.61\ (\times1.05)$ & $2.08\times10^{-09}\ (\times3)$
                % hsub=75nm
                & \cellcolor{grey_t} $21.19\ (\times1.04)$ & $7.04\times10^{-10}\ (\times2)$
                % hsub=100nm
                & \cellcolor{grey_t} $21.02\ (\times1.04)$ & $3.75\times10^{-10}\ (\times2)$ & 4 \\
        
        \hline 
       \fi 
    \end{NiceTabular} 
    }
\end{table*}


==> dummy/table5_color_final.tex <==

\begin{table*}[htp]
    \centering
   \caption{Process variation and MIV separation effect on transistor performance}\label{tab:process_variations}
   \scalebox{0.69}{
    \begin{NiceTabular}{|c|c|c|c|c|c|c|c|c|c|c|}
         \hline
          & $n_{src} $ & $n_{sub} $ & \multicolumn{2}{c|}{$H_{sub}=25 nm$}& \multicolumn{2}{c|}{$H_{sub}=50 nm$} & \multicolumn{2}{c|}{$H_{sub}=75 nm$}& \multicolumn{2}{c|}{$H_{sub}=100 nm$}  \\ \cline{4-11} 
        & $(cm^{-3})$ &  $(cm^{-3})$ & \multicolumn{1}{c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{c|}{$I_{leak} \ (A)$} 
        & \multicolumn{1}{c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{c|}{$I_{leak} \ (A)$}
        & \multicolumn{1}{c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{c|}{$I_{leak} \ (A)$}
        & \multicolumn{1}{c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{c|}{$I_{leak} \ (A)$} \\
        \hline 
        \multirow{8}{*}{\rotatebox{90}{$d_{sep}=50nm$}}
        & \multirow{2}{*}{1E18} 
    %   nsub % Imax_with_MIV % Ileak_withMIV
        & 1E15
                % hsub=25nm
               
                &  \cellcolor{red_t}  $4.60\ (\times1.30)$ & \cellcolor{red_t}  $1.65\times10^{-07}\ (\times171)$ 
                % hsub=50nm
                & \cellcolor{red_t}  $4.48\ (\times1.64)$ & \cellcolor{red_t}  $2.63\times10^{-07}\ (\times882)$
                % hsub=75nm
                & \cellcolor{red_t} $4.66\ (\times2.01)$ & \cellcolor{red_t}  $3.04\times10^{-07}\ (\times8090)$\cellcolor{red_t} 
                % hsub=100nm
                & \cellcolor{red_t} $4.55\ (\times2.53)$ & \cellcolor{red_t}  $3.50\times10^{-07}\ (\times68668)$ \\  \cline{3-11}
        
        & & 1E16
                % hsub=25nm
                & \cellcolor{red_t} $2.89\ (\times2.00)$ & \cellcolor{red_t}  $5.34\times10^{-09}\ (\times1865)$ 
                % hsub=50nm
                & \cellcolor{red_t} $1.71\ (\times3.30)$ & \cellcolor{red_t}  $1.01\times10^{-09}\ (\times13906)$
                % hsub=75nm
                & \cellcolor{red_t} $1.45\ (\times5.90)$ & \cellcolor{red_t}  $4.56\times10^{-10}\ (\times31241)$
                % hsub=100nm
                & \cellcolor{red_t} $1.30\ (\times6.53)$ & \cellcolor{red_t}  $3.10\times10^{-10}\ (\times44983)$  \\ \cline{4-11}
        

        \cline{2-3}
        & \multirow{2}{*}{1E19} 
        & 1E16   
                % hsub=25nm
                & \cellcolor{red_t} $11.89\ (\times1.29)$ & \cellcolor{red_t}  $8.93\times10^{-08}\ (\times442)$ 
                % hsub=50nm
                & \cellcolor{red_t}  $9.34\ (\times1.56)$ & \cellcolor{red_t}   $1.25\times10^{-08}\ (\times6988)$
                % hsub=75nm
                & \cellcolor{red_t} $8.23\ (\times1.84)$ & \cellcolor{red_t}  $5.00\times10^{-09}\ (\times18709)$
                % hsub=100nm
                & \cellcolor{red_t}  $7.92\ (\times1.90)$ & \cellcolor{red_t}  $2.83\times10^{-09}\ (\times31175)$   \\ \cline{3-11}
          
        
        & & 1E17
                % hsub=25nm
                & \cellcolor{red_t}   $8.57\ (\times1.33)$ & \cellcolor{red_t}  $1.78\times10^{-10}\ (\times244)$ 
                % hsub=50nm
                & \cellcolor{red_t}   $5.37\ (\times1.56)$ & \cellcolor{red_t}    $1.33\times10^{-12}\ (\times201)$
                % hsub=75nm
                & \cellcolor{red_t}  $4.51\ (\times1.59)$ & \cellcolor{red_t}  $4.61\times10^{-13}\ (\times99)$
                % hsub=100nm
                & \cellcolor{red_t}   $4.35\ (\times1.56)$ & \cellcolor{red_t}  $2.64\times10^{-13}\ (\times70)$ \\ \cline{4-11}
        
        

        \cline{2-3}
        & \multirow{2}{*}{1E20} 
        & 1E17   
                % hsub=25nm
                & \cellcolor{red_t} $30.60\ (\times1.12)$ & \cellcolor{red_t}  $8.23\times10^{-07}\ (\times7)$ 
                % hsub=50nm
                & \cellcolor{red_t}   $24.92\ (\times1.15)$ & \cellcolor{red_t}  $2.15\times10^{-08}\ (\times26)$
                % hsub=75nm
                &  \cellcolor{red_t}  $23.51\ (\times1.16)$ & \cellcolor{red_t}  $8.51\times10^{-09}\ (\times26)$
                % hsub=100nm
                &  \cellcolor{red_t}  $23.24\ (\times1.15)$ & \cellcolor{red_t}  $3.74\times10^{-09}\ (\times17)$  \\ \cline{3-11}
        
        & & 1E18 
                % hsub=25nm
                & \cellcolor{blue_t} $17.89\ (\times1.01)$ & \cellcolor{blue_t} $3.36\times10^{-11}\ (\times1.13)$ 
                % hsub=50nm
                &  \cellcolor{blue_t} $14.92\ (\times1.00)$ & \cellcolor{blue_t} $2.63\times10^{-12}\ (\times1.09)$
                % hsub=75nm
                & \cellcolor{blue_t} $14.81\ (\times1.01)$ & \cellcolor{blue_t} $2.35\times10^{-12}\ (\times1.21)$
                % hsub=100nm
                & \cellcolor{blue_t} $15.09\ (\times1.01)$ & \cellcolor{blue_t} $2.41\times10^{-12}\ (\times1.07)$ \\ \cline{4-11}
        
        \cline{2-3}
        
        & \multirow{2}{*}{1E21} 
        & 1E18   
                % hsub=25nm
                & \cellcolor{blue_t} $29.21\ (\times1.02)$ & \cellcolor{blue_t} $3.60\times10^{-08}\ (\times1.16)$ 
                % hsub=50nm
                & \cellcolor{blue_t} $24.61\ (\times1.02)$ & \cellcolor{blue_t} $2.37\times10^{-09}\ (\times1.20)$
                % hsub=75nm
                & \cellcolor{blue_t} $24.36\ (\times1.01)$ & \cellcolor{blue_t} $2.25\times10^{-09}\ (\times1.10)$
                % hsub=100nm
                & \cellcolor{blue_t} $24.93\ (\times1.01)$ & \cellcolor{blue_t} $3.60\times10^{-09}\ (\times1.09)$  \\ \cline{3-11}
        
        & & 1E19 
                % hsub=25nm
                & \cellcolor{blue_t} $4.01\ (\times1.03)$ & \cellcolor{blue_t} $3.79\times10^{-15}\ (\times1.16)$ 
                % hsub=50nm
                &  \cellcolor{blue_t}
                $4.01\ (\times1.02)$ & \cellcolor{blue_t} $4.45\times10^{-15}\ (\times1.13)$
                % hsub=75nm
                & \cellcolor{blue_t} $3.47\ (\times1.00)$ & \cellcolor{blue_t} $3.01\times10^{-15}\ (\times1.03)$
                % hsub=100nm
                & \cellcolor{blue_t} $4.32\ (\times1.00)$ & \cellcolor{blue_t} $6.39\times10^{-15}\ (\times1.00)$   \\ \cline{4-11}
        
        \hline 
    \end{NiceTabular} 
    }
\end{table*}









\begin{table}[htp]
    \centering
   \caption{KOZ recommendations based on M3D-IC process doping}\label{tab:process_KOZ}
   \scalebox{0.9}{
    \begin{NiceTabular}{|c|c|c|c|c|c|}
         \hline 
        $n_{src}$  &  $n_{sub}$ & \multicolumn{4}{c|}{$H_{sub}(nm)$} \\ \cline{3-6} 
          
         $(cm^{-3})$ &  $(cm^{-3})$ & {$25$}& {$50$} & {$75$}& {$100$} \\ 
          \hline
          \multirow{2}{*}{1E18}
          & 1E15
                % hsub=25nm % hsub=50nm % hsub=75nm % hsub=100nm
                & 400 & 450 & 500 & 500\\ \cline{2-6}
        & 1E16
                % hsub=25nm % hsub=50nm % hsub=75nm % hsub=100nm
                & 200 & 200 & 200 & 200 \\ \hline
                
                
          
          \multirow{2}{*}{1E19}
          & 1E16
                % hsub=25nm % hsub=50nm % hsub=75nm % hsub=100nm
                & 200 & 250 & 200 & 200 \\ \cline{2-6}
        & 1E17
                % hsub=25nm % hsub=50nm % hsub=75nm % hsub=100nm
                & 100 & 100 & 100 & 100\\ \hline
          
          
          \multirow{2}{*}{1E20}
          & 1E17
                % hsub=25nm % hsub=50nm % hsub=75nm % hsub=100nm
                & 100 & 100 & 100 & 100 \\ \cline{2-6}
        & 1E18
                % hsub=25nm % hsub=50nm % hsub=75nm % hsub=100nm
                & 50 & 50 & 50 & 50 \\ \hline
        \multirow{2}{*}{1E21}
          & 1E18
                % hsub=25nm % hsub=50nm % hsub=75nm % hsub=100nm
                & 50  & 50 & 50 & 50 \\ \cline{2-6}
        & 1E19
                % hsub=25nm % hsub=50nm % hsub=75nm % hsub=100nm
                & 50  & 50 & 50 & 50 \\ \hline
       
    \end{NiceTabular} 
    }
    

\end{table}


==> dummy/table5_with_color_backup.tex <==

\begin{table*}[htp]
    \centering
   \caption{Process variation and MIV separation effect on transistor performance}\label{tab:process_variations}
   \scalebox{0.69}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
         \hline
          & $n_{src} $ & $n_{sub} $ & \multicolumn{2}{c|}{$H_{sub}=25 nm$}& \multicolumn{2}{c|}{$H_{sub}=50 nm$} & \multicolumn{2}{c|}{$H_{sub}=75 nm$}& \multicolumn{2}{c|}{$H_{sub}=100 nm$}  \\ \cline{4-11} 
        & $(cm^{-3})$ &  $(cm^{-3})$ & \multicolumn{1}{c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{c|}{$I_{leak} \ (A)$} 
        & \multicolumn{1}{c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{c|}{$I_{leak} \ (A)$}
        & \multicolumn{1}{c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{c|}{$I_{leak} \ (A)$}
        & \multicolumn{1}{c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{c|}{$I_{leak} \ (A)$} \\
        \hline 
        \multirow{8}{*}{\rotatebox{90}{$d_{sep}=50nm$}}
        & \multirow{2}{*}{1E18} 
    %   nsub % Imax_with_MIV % Ileak_withMIV
        & 1E15
                % hsub=25nm
               
                &  $4.60\ (\times1.30)$ & $1.65\times10^{-07}\ (\times171)$ 
                % hsub=50nm
                & $4.48\ (\times1.64)$ & $2.63\times10^{-07}\ (\times882)$
                % hsub=75nm
                & $4.66\ (\times2.01)$ & $3.04\times10^{-07}\ (\times8090)$
                % hsub=100nm
                & $4.55\ (\times2.53)$ & $3.50\times10^{-07}\ (\times68668)$ \\  \cline{3-11}
        
        & & 1E16
                % hsub=25nm
                & $2.89\ (\times2.00)$ &  $5.34\times10^{-09}\ (\times1865)$ 
                % hsub=50nm
                & $1.71\ (\times3.30)$ &  $1.01\times10^{-09}\ (\times13906)$
                % hsub=75nm
                & $1.45\ (\times5.90)$ &  $4.56\times10^{-10}\ (\times31241)$
                % hsub=100nm
                & $1.30\ (\times6.53)$ &  $3.10\times10^{-10}\ (\times44983)$  \\ \cline{4-11}
        

        \cline{2-3}
        & \multirow{2}{*}{1E19} 
        & 1E16   
                % hsub=25nm
                & $11.89\ (\times1.29)$ &  $8.93\times10^{-08}\ (\times442)$ 
                % hsub=50nm
                & $9.34\ (\times1.56)$ &  $1.25\times10^{-08}\ (\times6988)$
                % hsub=75nm
                & $8.23\ (\times1.84)$ &  $5.00\times10^{-09}\ (\times18709)$
                % hsub=100nm
                & $7.92\ (\times1.90)$ &  $2.83\times10^{-09}\ (\times31175)$   \\ \cline{3-11}
          
        
        & & 1E17
                % hsub=25nm
                &   $8.57\ (\times1.33)$ &  $1.78\times10^{-10}\ (\times244)$ 
                % hsub=50nm
                &  $5.37\ (\times1.56)$ &   $1.33\times10^{-12}\ (\times201)$
                % hsub=75nm
                &  $4.51\ (\times1.59)$ &  $4.61\times10^{-13}\ (\times99)$
                % hsub=100nm
                &  $4.35\ (\times1.56)$ &  $2.64\times10^{-13}\ (\times70)$ \\ \cline{4-11}
        
        

        \cline{2-3}
        & \multirow{2}{*}{1E20} 
        & 1E17   
                % hsub=25nm
                &  $30.60\ (\times1.12)$ & $8.23\times10^{-07}\ (\times7)$ 
                % hsub=50nm
                &  $24.92\ (\times1.15)$ & $2.15\times10^{-08}\ (\times26)$
                % hsub=75nm
                &  $23.51\ (\times1.16)$ & $8.51\times10^{-09}\ (\times26)$
                % hsub=100nm
                &  $23.24\ (\times1.15)$ & $3.74\times10^{-09}\ (\times17)$  \\ \cline{3-11}
        
        & & 1E18 
                % hsub=25nm
                &  $17.89\ (\times1.01)$ &  $3.36\times10^{-11}\ (\times1.13)$ 
                % hsub=50nm
                &   $14.92\ (\times1.00)$ &  $2.63\times10^{-12}\ (\times1.09)$
                % hsub=75nm
                &  $14.81\ (\times1.01)$ &  $2.35\times10^{-12}\ (\times1.21)$
                % hsub=100nm
                &  $15.09\ (\times1.01)$ &  $2.41\times10^{-12}\ (\times1.07)$ \\ \cline{4-11}
        
        \cline{2-3}
        
        & \multirow{2}{*}{1E21} 
        & 1E18   
                % hsub=25nm
                & $29.21\ (\times1.02)$ &  $3.60\times10^{-08}\ (\times1.16)$ 
                % hsub=50nm
                &  $24.61\ (\times1.02)$ &  $2.37\times10^{-09}\ (\times1.20)$
                % hsub=75nm
                &  $24.36\ (\times1.01)$ &  $2.25\times10^{-09}\ (\times1.10)$
                % hsub=100nm
                &  $24.93\ (\times1.01)$ &  $3.60\times10^{-09}\ (\times1.09)$  \\ \cline{3-11}
        
        & & 1E19 
                % hsub=25nm
                & $4.01\ (\times1.03)$ &  $3.79\times10^{-15}\ (\times1.16)$ 
                % hsub=50nm
                &  $4.01\ (\times1.02)$ &  $4.45\times10^{-15}\ (\times1.13)$
                % hsub=75nm
                &  $3.47\ (\times1.00)$ &  $3.01\times10^{-15}\ (\times1.03)$
                % hsub=100nm
                &  $4.32\ (\times1.00)$ &  $6.39\times10^{-15}\ (\times1.00)$   \\ \cline{4-11}
        
        \hline 
        
        \iffalse
        \hline
        
        \multirow{5}{*}{\rotatebox{90}{$d_{sep}=100nm$}}
        & \multirow{2}{*}{1E18} 
    %   nsub % Imax_with_MIV % Ileak_withMIV
        & 1E15
                % hsub=25nm
                &  $4.31\ (\times1.22)$ & $4.54\times10^{-08}\ (\times47)$ 
                % hsub=50nm
                & $4.02\ (\times1.47)$ &  $7.08\times10^{-08}\ (\times237)$
                % hsub=75nm
                & $4.00\ (\times1.72)$ & $7.40\times10^{-08}\ (\times1971)$
                % hsub=100nm
                & $3.84\ (\times2.13)$ & $8.07\times10^{-08}\ (\times15839)$ & 1 \\ \cline{3-12}
        
        & & 1E16
                % hsub=25nm
                & $2.48\ (\times1.72)$ &  $3.51\times10^{-10}\ (\times123)$ 
                % hsub=50nm
                & $1.22\ (\times2.36)$ &  $2.94\times10^{-11}\ (\times403)$
                % hsub=75nm
                & $0.89\ (\times3.62)$ &  $6.35\times10^{-12}\ (\times435)$
                % hsub=100nm
                & $0.73\ (\times3.66)$ &  $2.78\times10^{-12}\ (\times404)$ & \multirow{2}{*}{2} \\ 
                \cline{4-11}
        

        
        \cline{2-3}
        & \multirow{2}{*}{1E19} 
        & 1E16   
                % hsub=25nm
                & $11.23\ (\times1.22)$ &  $1.23\times10^{-08}\ (\times61)$ 
                % hsub=50nm
                & $8.24\ (\times1.37)$ &  $5.11\times10^{-10}\ (\times285)$
                % hsub=75nm
                & $6.86\ (\times1.54)$ &  $8.28\times10^{-11}\ (\times310)$
                % hsub=100nm
                & $6.43\ (\times1.54)$ &  $2.75\times10^{-11}\ (\times303)$ &  \\ \cline{3-12}
          
        % edit from here
        & & 1E17
                % hsub=25nm
                &   $7.33\ (\times1.13)$ &  $2.84\times10^{-12}\ (\times4)$ 
                % hsub=50nm
                &  $3.76\ (\times1.09)$ &  $1.32\times10^{-14}\ (\times2)$
                % hsub=75nm
                &  $3.15\ (\times1.12)$ &  $7.01\times10^{-15}\ (\times2)$
                % hsub=100nm
                &  $3.01\ (\times1.08)$ &  $5.31\times10^{-15}\ (\times1.41)$ & 3 \\ \cline{3-12}
        

        \cline{2-11}
        & \multirow{1}{*}{1E20} 
        & 1E17   
                % hsub=25nm
                &  $28.87\ (\times1.06)$ & $2.79\times10^{-07}\ (\times2)$ 
                % hsub=50nm
                &  $22.61\ (\times1.05)$ & $2.08\times10^{-09}\ (\times3)$
                % hsub=75nm
                &  $21.19\ (\times1.04)$ & $7.04\times10^{-10}\ (\times2)$
                % hsub=100nm
                &  $21.02\ (\times1.04)$ & $3.75\times10^{-10}\ (\times2)$ & 4 \\
        
        \hline 
       \fi 
       
    \end{tabular} 
    }
\end{table*}









\begin{table}[htp]
    \centering
   \caption{Process variation and MIV separation effect on transistor performance}\label{tab:process_KOZ}
   \scalebox{0.78}{
    \begin{NiceTabular}{|c|c|c|c|c|c|}
         \hline
          $n_{src} $ & $n_{sub} $ & {$H_{sub}=25 nm$}& {$H_{sub}=50 nm$} & {$H_{sub}=75 nm$}& {$H_{sub}=100 nm$} \\ 
          \hline
          \multirow{2}{*}{1E18}
          & 1E15
                % hsub=25nm % hsub=50nm % hsub=75nm % hsub=100nm
                & 400 & 450 & 500 & 500\\ \cline{2-6}
        & 1E16
                % hsub=25nm % hsub=50nm % hsub=75nm % hsub=100nm
                & 200 & 200 & 200 & 200 \\ \hline
                
                
          
          \multirow{2}{*}{1E19}
          & 1E16
                % hsub=25nm % hsub=50nm % hsub=75nm % hsub=100nm
                & 200 & 250 & 200 & 200 \\ \cline{2-6}
        & 1E17
                % hsub=25nm % hsub=50nm % hsub=75nm % hsub=100nm
                & 100 & 100 & 100 & 100\\ \hline
          
          
          \multirow{2}{*}{1E20}
          & 1E17
                % hsub=25nm % hsub=50nm % hsub=75nm % hsub=100nm
                & 100 & 100 & 100 & 100 \\ \cline{2-6}
        & 1E18
                % hsub=25nm % hsub=50nm % hsub=75nm % hsub=100nm
                & 50 & 50 & 50 & 50 \\ \hline
        \multirow{2}{*}{1E21}
          & 1E18
                % hsub=25nm % hsub=50nm % hsub=75nm % hsub=100nm
                & 50  & 50 & 50 & 50 \\ \cline{2-6}
        & 1E19
                % hsub=25nm % hsub=50nm % hsub=75nm % hsub=100nm
                & 50  & 50 & 50 & 50 \\ \hline
            
          
          
       
    \end{NiceTabular} 
    }
    

\end{table}


==> dummy/table_v2.tex <==

\begin{table*}[htp]
    \centering
   \caption{Process variation and MIV separation effect on transistor performance}\label{tab:process_variations}
   \scalebox{0.65}{
    \begin{NiceTabular}{|c|c|c|l|l|l|l|l|l|l|l|c|}
         \hline
          & $n_{src} $ & $n_{sub} $ & \multicolumn{2}{c|}{$H_{sub}=25 nm$}& \multicolumn{2}{c|}{$H_{sub}=50 nm$} & \multicolumn{2}{c|}{$H_{sub}=75 nm$}& \multicolumn{2}{c|}{$H_{sub}=100 nm$} & \multirow{2}{*}{Case} \\ \cline{4-11} 
        \textbf {} & $(cm^{-3})$ &  $(cm^{-3})$ & \multicolumn{1}{|c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{|c|}{$I_{leak} \ (A)$} 
        & \multicolumn{1}{|c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{|c|}{$I_{leak} \ (A)$}
        & \multicolumn{1}{|c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{|c|}{$I_{leak} \ (A)$}
        & \multicolumn{1}{|c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{|c|}{$I_{leak} \ (A)$} & \\
        \hline 
        \multirow{8}{*}{\rotatebox{90}{$d_{sep}=50nm$}}
        & \multirow{2}{*}{1E18} 
    %   nsub % Imax_with_MIV % Ileak_withMIV
        & 1E15
                % hsub=25nm
               
                &  \bc $4.60\ (\times1.30)$ & \bc $1.65\times10^{-07}\ (\times171)$ 
                % hsub=50nm
                & \bc $4.48\ (\times1.64)$ & \bc $2.63\times10^{-07}\ (\times882)$
                % hsub=75nm
                & \bc $4.66\ (\times2.01)$ & \bc $3.04\times10^{-07}\ (\times8090)$
                % hsub=100nm
                & \bc $4.55\ (\times2.53)$ & \bc $3.50\times10^{-07}\ (\times68668)$  & 1 \\ \cline{3-12}
        
        & & 1E16
                % hsub=25nm
                & $2.89\ (\times2.00)$ & \cellcolor{green_t} $5.34\times10^{-09}\ (\times1865)$ 
                % hsub=50nm
                & $1.71\ (\times3.30)$ & \cellcolor{green_t} $1.01\times10^{-09}\ (\times13906)$
                % hsub=75nm
                & $1.45\ (\times5.90)$ & \cellcolor{green_t} $4.56\times10^{-10}\ (\times31241)$
                % hsub=100nm
                & $1.30\ (\times6.53)$ & \cellcolor{green_t} $3.10\times10^{-10}\ (\times44983)$ & \multirow{2}{*}{2} \\ \cline{4-11}
        

        \cline{2-3}
        & \multirow{2}{*}{1E19} 
        & 1E16   
                % hsub=25nm
                & $11.89\ (\times1.29)$ & \cellcolor{green_t} $8.93\times10^{-08}\ (\times442)$ 
                % hsub=50nm
                & $9.34\ (\times1.56)$ & \cellcolor{green_t} $1.25\times10^{-08}\ (\times6988)$
                % hsub=75nm
                & $8.23\ (\times1.84)$ & \cellcolor{green_t} $5.00\times10^{-09}\ (\times18709)$
                % hsub=100nm
                & $7.92\ (\times1.90)$ & \cellcolor{green_t} $2.83\times10^{-09}\ (\times31175)$ &  \\ \cline{3-12}
          
        
        & & 1E17
                % hsub=25nm
                &  \pc $8.57\ (\times1.33)$ & \pc $1.78\times10^{-10}\ (\times244)$ 
                % hsub=50nm
                & \pc $5.37\ (\times1.56)$ &  \pc $1.33\times10^{-12}\ (\times201)$
                % hsub=75nm
                & \pc $4.51\ (\times1.59)$ & \pc $4.61\times10^{-13}\ (\times99)$
                % hsub=100nm
                & \pc $4.35\ (\times1.56)$ & \pc $2.64\times10^{-13}\ (\times70)$ & 3 \\ \cline{4-12}
        
        

        \cline{2-3}
        & \multirow{2}{*}{1E20} 
        & 1E17   
                % hsub=25nm
                & \cellcolor{grey_t} $30.60\ (\times1.12)$ & $8.23\times10^{-07}\ (\times7)$ 
                % hsub=50nm
                & \cellcolor{grey_t} $24.92\ (\times1.15)$ & $2.15\times10^{-08}\ (\times26)$
                % hsub=75nm
                & \cellcolor{grey_t} $23.51\ (\times1.16)$ & $8.51\times10^{-09}\ (\times26)$
                % hsub=100nm
                & \cellcolor{grey_t} $23.24\ (\times1.15)$ & $3.74\times10^{-09}\ (\times17)$ & 4 \\ \cline{3-12}
        
        & & 1E18 
                % hsub=25nm
                & \yc $17.89\ (\times1.01)$ & \yc $3.36\times10^{-11}\ (\times1.13)$ 
                % hsub=50nm
                & \yc  $14.92\ (\times1.00)$ & \yc $2.63\times10^{-12}\ (\times1.09)$
                % hsub=75nm
                & \yc $14.81\ (\times1.01)$ & \yc $2.35\times10^{-12}\ (\times1.21)$
                % hsub=100nm
                & \yc $15.09\ (\times1.01)$ & \yc $2.41\times10^{-12}\ (\times1.07)$ & \multirow{3}{*}{5}\\ \cline{4-11}
        
        \cline{2-3}
        
        & \multirow{2}{*}{1E21} 
        & 1E18   
                % hsub=25nm
                & \yc $29.21\ (\times1.02)$ & \yc $3.60\times10^{-08}\ (\times1.16)$ 
                % hsub=50nm
                & \yc $24.61\ (\times1.02)$ & \yc $2.37\times10^{-09}\ (\times1.20)$
                % hsub=75nm
                & \yc $24.36\ (\times1.01)$ & \yc $2.25\times10^{-09}\ (\times1.10)$
                % hsub=100nm
                & \yc $24.93\ (\times1.01)$ & \yc $3.60\times10^{-09}\ (\times1.09)$ &  \\ \cline{3-11}
        
        & & 1E19 
                % hsub=25nm
                & \yc $4.01\ (\times1.03)$ & \yc $3.79\times10^{-15}\ (\times1.16)$ 
                % hsub=50nm
                & \yc $4.01\ (\times1.02)$ & \yc $4.45\times10^{-15}\ (\times1.13)$
                % hsub=75nm
                & \yc $3.47\ (\times1.00)$ & \yc $3.01\times10^{-15}\ (\times1.03)$
                % hsub=100nm
                & \yc $4.32\ (\times1.00)$ & \yc $6.39\times10^{-15}\ (\times1.00)$ &  \\ \cline{4-12}
        

        
        \hline \hline
        
        \multirow{5}{*}{\rotatebox{90}{$d_{sep}=100nm$}}
        & \multirow{2}{*}{1E18} 
    %   nsub % Imax_with_MIV % Ileak_withMIV
        & 1E15
                % hsub=25nm
                &  \bc $4.31\ (\times1.22)$ & \bc $4.54\times10^{-08}\ (\times47)$ 
                % hsub=50nm
                & \bc $4.02\ (\times1.47)$ &  \bc $7.08\times10^{-08}\ (\times237)$
                % hsub=75nm
                & \bc $4.00\ (\times1.72)$ & \bc $7.40\times10^{-08}\ (\times1971)$
                % hsub=100nm
                & \bc $3.84\ (\times2.13)$ & \bc $8.07\times10^{-08}\ (\times15839)$ & 1 \\ \cline{3-12}
        
        & & 1E16
                % hsub=25nm
                & $2.48\ (\times1.72)$ & \cellcolor{green_t} $3.51\times10^{-10}\ (\times123)$ 
                % hsub=50nm
                & $1.22\ (\times2.36)$ & \cellcolor{green_t} $2.94\times10^{-11}\ (\times403)$
                % hsub=75nm
                & $0.89\ (\times3.62)$ & \cellcolor{green_t} $6.35\times10^{-12}\ (\times435)$
                % hsub=100nm
                & $0.73\ (\times3.66)$ & \cellcolor{green_t} $2.78\times10^{-12}\ (\times404)$ & \multirow{2}{*}{2} \\ 
                \cline{4-11}
        

        
        \cline{2-3}
        & \multirow{2}{*}{1E19} 
        & 1E16   
                % hsub=25nm
                & $11.23\ (\times1.22)$ & \cellcolor{green_t} $1.23\times10^{-08}\ (\times61)$ 
                % hsub=50nm
                & $8.24\ (\times1.37)$ & \cellcolor{green_t} $5.11\times10^{-10}\ (\times285)$
                % hsub=75nm
                & $6.86\ (\times1.54)$ & \cellcolor{green_t} $8.28\times10^{-11}\ (\times310)$
                % hsub=100nm
                & $6.43\ (\times1.54)$ & \cellcolor{green_t} $2.75\times10^{-11}\ (\times303)$ &  \\ \cline{3-12}
          
        % edit from here
        & & 1E17
                % hsub=25nm
                &  \pc $7.33\ (\times1.13)$ & \pc $2.84\times10^{-12}\ (\times4)$ 
                % hsub=50nm
                & \pc $3.76\ (\times1.09)$ & \pc $1.32\times10^{-14}\ (\times2)$
                % hsub=75nm
                & \pc $3.15\ (\times1.12)$ & \pc $7.01\times10^{-15}\ (\times2)$
                % hsub=100nm
                & \pc $3.01\ (\times1.08)$ & \pc $5.31\times10^{-15}\ (\times1.41)$ & 3\\ \cline{3-12}
        

        \cline{2-11}
        & \multirow{1}{*}{1E20} 
        & 1E17   
                % hsub=25nm
                & \cellcolor{grey_t} $28.87\ (\times1.06)$ & $2.79\times10^{-07}\ (\times2)$ 
                % hsub=50nm
                & \cellcolor{grey_t} $22.61\ (\times1.05)$ & $2.08\times10^{-09}\ (\times3)$
                % hsub=75nm
                & \cellcolor{grey_t} $21.19\ (\times1.04)$ & $7.04\times10^{-10}\ (\times2)$
                % hsub=100nm
                & \cellcolor{grey_t} $21.02\ (\times1.04)$ & $3.75\times10^{-10}\ (\times2)$ & 4 \\
        
        \hline 
        
    \end{NiceTabular}
 }   
\end{table*}




% with case 

\begin{table*}[htp]
    \centering
   \caption{Process variation and MIV separation effect on transistor performance}\label{tab:process_variations}
   \scalebox{0.65}{
    \begin{NiceTabular}{|c|c|c|l|l|l|l|l|l|l|l|c|}
         \hline
          & $n_{src} $ & $n_{sub} $ & \multicolumn{2}{c|}{$H_{sub}=25 nm$}& \multicolumn{2}{c|}{$H_{sub}=50 nm$} & \multicolumn{2}{c|}{$H_{sub}=75 nm$}& \multicolumn{2}{c|}{$H_{sub}=100 nm$} & \multirow{2}{*}{Case} \\ \cline{4-11} 
        \textbf {} & $(cm^{-3})$ &  $(cm^{-3})$ & \multicolumn{1}{|c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{|c|}{$I_{leak} \ (A)$} 
        & \multicolumn{1}{|c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{|c|}{$I_{leak} \ (A)$}
        & \multicolumn{1}{|c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{|c|}{$I_{leak} \ (A)$}
        & \multicolumn{1}{|c|}{$I_{max} \ (\mu  A)$} & \multicolumn{1}{|c|}{$I_{leak} \ (A)$} & \\
        \hline 
        \multirow{8}{*}{\rotatebox{90}{$d_{sep}=50nm$}}
        & \multirow{2}{*}{1E18} 
    %   nsub % Imax_with_MIV % Ileak_withMIV
        & 1E15
                % hsub=25nm
               
                &  $4.60\ (\times1.30)$ & $1.65\times10^{-07}\ (\times171)$ 
                % hsub=50nm
                & $4.48\ (\times1.64)$ & $2.63\times10^{-07}\ (\times882)$
                % hsub=75nm
                & $4.66\ (\times2.01)$ & $3.04\times10^{-07}\ (\times8090)$
                % hsub=100nm
                & $4.55\ (\times2.53)$ & $3.50\times10^{-07}\ (\times68668)$  & 1 \\ \cline{3-12}
        
        & & 1E16
                % hsub=25nm
                & $2.89\ (\times2.00)$ &  $5.34\times10^{-09}\ (\times1865)$ 
                % hsub=50nm
                & $1.71\ (\times3.30)$ &  $1.01\times10^{-09}\ (\times13906)$
                % hsub=75nm
                & $1.45\ (\times5.90)$ &  $4.56\times10^{-10}\ (\times31241)$
                % hsub=100nm
                & $1.30\ (\times6.53)$ &  $3.10\times10^{-10}\ (\times44983)$ & \multirow{2}{*}{2} \\ \cline{4-11}
        

        \cline{2-3}
        & \multirow{2}{*}{1E19} 
        & 1E16   
                % hsub=25nm
                & $11.89\ (\times1.29)$ &  $8.93\times10^{-08}\ (\times442)$ 
                % hsub=50nm
                & $9.34\ (\times1.56)$ &  $1.25\times10^{-08}\ (\times6988)$
                % hsub=75nm
                & $8.23\ (\times1.84)$ &  $5.00\times10^{-09}\ (\times18709)$
                % hsub=100nm
                & $7.92\ (\times1.90)$ &  $2.83\times10^{-09}\ (\times31175)$ &  \\ \cline{3-12}
          
        
        & & 1E17
                % hsub=25nm
                &   $8.57\ (\times1.33)$ &  $1.78\times10^{-10}\ (\times244)$ 
                % hsub=50nm
                &  $5.37\ (\times1.56)$ &   $1.33\times10^{-12}\ (\times201)$
                % hsub=75nm
                &  $4.51\ (\times1.59)$ &  $4.61\times10^{-13}\ (\times99)$
                % hsub=100nm
                &  $4.35\ (\times1.56)$ &  $2.64\times10^{-13}\ (\times70)$ & 3 \\ \cline{4-12}
        
        

        \cline{2-3}
        & \multirow{2}{*}{1E20} 
        & 1E17   
                % hsub=25nm
                &  $30.60\ (\times1.12)$ & $8.23\times10^{-07}\ (\times7)$ 
                % hsub=50nm
                &  $24.92\ (\times1.15)$ & $2.15\times10^{-08}\ (\times26)$
                % hsub=75nm
                &  $23.51\ (\times1.16)$ & $8.51\times10^{-09}\ (\times26)$
                % hsub=100nm
                &  $23.24\ (\times1.15)$ & $3.74\times10^{-09}\ (\times17)$ & 4 \\ \cline{3-12}
        
        & & 1E18 
                % hsub=25nm
                &  $17.89\ (\times1.01)$ &  $3.36\times10^{-11}\ (\times1.13)$ 
                % hsub=50nm
                &   $14.92\ (\times1.00)$ &  $2.63\times10^{-12}\ (\times1.09)$
                % hsub=75nm
                &  $14.81\ (\times1.01)$ &  $2.35\times10^{-12}\ (\times1.21)$
                % hsub=100nm
                &  $15.09\ (\times1.01)$ &  $2.41\times10^{-12}\ (\times1.07)$ & \multirow{3}{*}{5}\\ \cline{4-11}
        
        \cline{2-3}
        
        & \multirow{2}{*}{1E21} 
        & 1E18   
                % hsub=25nm
                &  $29.21\ (\times1.02)$ &  $3.60\times10^{-08}\ (\times1.16)$ 
                % hsub=50nm
                &  $24.61\ (\times1.02)$ &  $2.37\times10^{-09}\ (\times1.20)$
                % hsub=75nm
                &  $24.36\ (\times1.01)$ &  $2.25\times10^{-09}\ (\times1.10)$
                % hsub=100nm
                &  $24.93\ (\times1.01)$ &  $3.60\times10^{-09}\ (\times1.09)$ &  \\ \cline{3-11}
        
        & & 1E19 
                % hsub=25nm
                &  $4.01\ (\times1.03)$ &  $3.79\times10^{-15}\ (\times1.16)$ 
                % hsub=50nm
                &  $4.01\ (\times1.02)$ &  $4.45\times10^{-15}\ (\times1.13)$
                % hsub=75nm
                &  $3.47\ (\times1.00)$ &  $3.01\times10^{-15}\ (\times1.03)$
                % hsub=100nm
                &  $4.32\ (\times1.00)$ &  $6.39\times10^{-15}\ (\times1.00)$ &  \\ \cline{4-12}
        

        
        \hline 
        
        \iffalse
        \hline
        
        \multirow{5}{*}{\rotatebox{90}{$d_{sep}=100nm$}}
        & \multirow{2}{*}{1E18} 
    %   nsub % Imax_with_MIV % Ileak_withMIV
        & 1E15
                % hsub=25nm
                &  $4.31\ (\times1.22)$ & $4.54\times10^{-08}\ (\times47)$ 
                % hsub=50nm
                & $4.02\ (\times1.47)$ &  $7.08\times10^{-08}\ (\times237)$
                % hsub=75nm
                & $4.00\ (\times1.72)$ & $7.40\times10^{-08}\ (\times1971)$
                % hsub=100nm
                & $3.84\ (\times2.13)$ & $8.07\times10^{-08}\ (\times15839)$ & 1 \\ \cline{3-12}
        
        & & 1E16
                % hsub=25nm
                & $2.48\ (\times1.72)$ &  $3.51\times10^{-10}\ (\times123)$ 
                % hsub=50nm
                & $1.22\ (\times2.36)$ &  $2.94\times10^{-11}\ (\times403)$
                % hsub=75nm
                & $0.89\ (\times3.62)$ &  $6.35\times10^{-12}\ (\times435)$
                % hsub=100nm
                & $0.73\ (\times3.66)$ &  $2.78\times10^{-12}\ (\times404)$ & \multirow{2}{*}{2} \\ 
                \cline{4-11}
        

        
        \cline{2-3}
        & \multirow{2}{*}{1E19} 
        & 1E16   
                % hsub=25nm
                & $11.23\ (\times1.22)$ &  $1.23\times10^{-08}\ (\times61)$ 
                % hsub=50nm
                & $8.24\ (\times1.37)$ &  $5.11\times10^{-10}\ (\times285)$
                % hsub=75nm
                & $6.86\ (\times1.54)$ &  $8.28\times10^{-11}\ (\times310)$
                % hsub=100nm
                & $6.43\ (\times1.54)$ &  $2.75\times10^{-11}\ (\times303)$ &  \\ \cline{3-12}
          
        % edit from here
        & & 1E17
                % hsub=25nm
                &   $7.33\ (\times1.13)$ &  $2.84\times10^{-12}\ (\times4)$ 
                % hsub=50nm
                &  $3.76\ (\times1.09)$ &  $1.32\times10^{-14}\ (\times2)$
                % hsub=75nm
                &  $3.15\ (\times1.12)$ &  $7.01\times10^{-15}\ (\times2)$
                % hsub=100nm
                &  $3.01\ (\times1.08)$ &  $5.31\times10^{-15}\ (\times1.41)$ & 3 \\ \cline{3-12}
        

        \cline{2-11}
        & \multirow{1}{*}{1E20} 
        & 1E17   
                % hsub=25nm
                &  $28.87\ (\times1.06)$ & $2.79\times10^{-07}\ (\times2)$ 
                % hsub=50nm
                &  $22.61\ (\times1.05)$ & $2.08\times10^{-09}\ (\times3)$
                % hsub=75nm
                &  $21.19\ (\times1.04)$ & $7.04\times10^{-10}\ (\times2)$
                % hsub=100nm
                &  $21.02\ (\times1.04)$ & $3.75\times10^{-10}\ (\times2)$ & 4 \\
        
        \hline 
       \fi 
    \end{NiceTabular} 
    }
\end{table*}




